(Dis)Proving Spectre Security with Speculation-Passing Style

Constant-time (CT) verification tools are commonly used for detecting potential side-channel vulnerabilities in cryptographic libraries. Recently, a new class of tools, called speculative constant-time (SCT) tools, has also been used for detecting potential Spectre vulnerabilities. In many cases, these SCT tools have emerged as liftings of CT tools. However, these liftings are seldom defined precisely and are almost never analyzed formally. The goal of this paper is to address this gap, by developing formal foundations for these liftings, and to demonstrate that these foundations can yield practical benefits. Concretely, we introduce a program transformation, coined Speculation-Passing Style (SPS), for reducing SCT verification to CT verification. Essentially, the transformation instruments the program with a new input that corresponds to attacker-controlled predictions and modifies the program to follow them. This approach is sound and complete, in the sense that a program is SCT if and only if its SPS transform is CT. Thus, we can leverage existing CT verification tools to prove SCT; we illustrate this by combining SPS with three standard methodologies for CT verification, namely reducing it to non-interference, assertion safety and dynamic taint analysis. We realize these combinations with three existing tools, EasyCrypt, BINSEC, and ctgrind, and we evaluate them on Kocher's benchmarks for Spectre-v1. Our results focus on Spectre-v1 in the standard CT leakage model; however, we also discuss applications of our method to other variants of Spectre and other leakage models.

==> Makefile <==
NJOBS ?= 2
MAKEFLAGS += --jobs=$(NJOBS)

REFS ?= bib.bib
MAIN ?= dedsct

DIROUTPUT ?= latex_output

CMDTEX = \
	pdflatex \
	-synctex=1 \
	-halt-on-error -interaction=nonstopmode \
	-output-directory $(DIROUTPUT)
CMDBIB = bibtex

SOURCES = \
	$(wildcard *.tex) $(wildcard *.sty) $(wildcard *.bib) \
	$(wildcard fig/*) $(wildcard img/*)

.PHONY: all clean lint

all: $(MAIN).pdf

$(DIROUTPUT):
	mkdir -p "$(DIROUTPUT)"

%.pdf: %.tex $(SOURCES) | $(DIROUTPUT)
	$(CMDTEX) "$<"
	if [ -f "$(DIROUTPUT)/$*.aux" ] && grep -q '\\bibdata' "$(DIROUTPUT)/$*.aux"; then \
	  $(CMDBIB) "$(DIROUTPUT)/$*"; \
	  $(CMDTEX) "$<"; \
	fi
	$(CMDTEX) "$<"
	cp "$(DIROUTPUT)/$@" .

clean:
	rm -rvf "$(DIROUTPUT)" "$(MAIN).pdf"

lint:
	chktex "$(MAIN).tex" || true
	lacheck "$(MAIN).tex" || true
	@if [ -f "$(DIROUTPUT)/$(MAIN).aux" ]; then \
		checkcites "$(DIROUTPUT)/$(MAIN).aux"; \
	fi || true
	@if [ -f "$(REFS)" ]; then bibformat "$(REFS)"; fi || true

